How does Docker affect energy consumption? Evaluating workloads in and out of Docker containers

Context: Virtual machines provide isolation of services at the cost of hypervisors and more resource usage. This spurred the growth of systems like Docker that enable single hosts to isolate several applications, similar to VMs, within a low-overhead abstraction called containers. Motivation: Although containers tout low overhead performance, do they still have low energy consumption? Methodology: This work statistically compares ($t$-test, Wilcoxon) the energy consumption of three application workloads in Docker and on bare-metal Linux. Results: In all cases, there was a statistically significant ($t$-test and Wilcoxon $p < 0.05$) increase in energy consumption when running tests in Docker, mostly due to the performance of I/O system calls.

==> sections/future_work.tex <==
\section{Future Work}
\label{sec:future-work}

\todo{Write any and all future work.}

